Explaining Chest X-ray Pathologies in Natural Language

Most deep learning algorithms lack explanations for their predictions, which limits their deployment in clinical practice. Approaches to improve explainability, especially in medical imaging, have often been shown to convey limited information, be overly reassuring, or lack robustness. In this work, we introduce the task of generating natural language explanations (NLEs) to justify predictions made on medical images. NLEs are human-friendly and comprehensive, and enable the training of intrinsically explainable models. To this goal, we introduce MIMIC-NLE, the first, large-scale, medical imaging dataset with NLEs. It contains over 38,000 NLEs, which explain the presence of various thoracic pathologies and chest X-ray findings. We propose a general approach to solve the task and evaluate several architectures on this dataset, including via clinician assessment.

==> sections/related_work.tex <==
\subsubsection{Natural Language Explanations.}

NLEs aim to explain the decision-making process of a model via generated sentences. They are motivated by their user-friendliness in explaining model decisions to humans and by their ability to convey complex reasoning. This addresses the shortcomings of the more common extractive rationales, i.e. identifying meaningful subsets of the input, which can be hard to understand, even for expert users \cite{alufaisan_does_2021, kaur_interpreting_2020}.

% existing work
% Besides early adoptions of textual explanations for traditional AI \cite{core_building_2006, lane_explainable_2005, shortliffe_model_1975}, 
% NLEs for deep learning models have first been adopted in vision \cite{hendricks_generating_2016}. Most NLE approaches consist of a task model $M_T$ and an explanation generator $M_E$. $M_T$ is used to solve the task at hand (e.g. Natural Language Inference (NLI) \cite{bowman_large_2015}) and $M_E$ generates an explanation conditioned on the representation that $M_T$ learned to solve the task. Generally, existing work differentiates between first answering the task and condition the explanation on the answer (\emph{predict-then-explain}) or first generating an explanation and extracting the answer from that (\emph{explain-then-predict}) \cite{camburu_e-snli_2018}. 
NLEs are most commonly applied in NLP problems \cite{camburu_e-snli_2018, majumder_rationale-inspired_2021, bhagavatula_abductive_2019, atanasova_generating_2020, kotonya_explainable_2020, narang_wt5_2020, kumar_nile_2020, rajani_explain_2019}. NLE architectures generally consist of a task model $M_T$ and an explanation generator $M_E$. $M_T$ is used to solve the task at hand (e.g. Natural Language Inference (NLI) \cite{bowman_large_2015}) and $M_E$ generates an explanation conditioned on the representation that $M_T$ learned to solve the task. \cite{camburu_e-snli_2018} propose two recurrent neural networks (RNNs), one as $M_T$ for an NLI task and one as $M_T$ to provide NLEs that explain the answer. Recent work also includes WT5 \cite{narang_wt5_2020}, where they train a text-to-text model to both solve the task and generate the explanation, and \cite{majumder_rationale-inspired_2021}, who generate NLEs based on extractive rationales and commonsense knowledge. There has also been growing interest in NLEs for vision task. A recent benchmark compares four architectures that provide NLEs for vision-language tasks \cite{kayser_e-vil_2021}. The results show that transformer-based architectures, such as a combination of UNITER \cite{chen_uniter_2020} and GPT-2 \cite{radford_language_nodate}, outperform RNN-based methods such as PJ-X \cite{park_multimodal_2018}. We leverage the findings from this work and propose X-rayner, a self-explainable model for chest x-ray classification.  
In order to facilitate supervised training of NLEs there have also been numberous efforts to build NLE datasets. \cite{camburu_e-snli_2018} and \cite{zellers_recognition_2019-1} hire crowd workers to annotate NLEs to an NLI and VQA dataset, respectively. e-SNLI-VE \cite{kayser_e-vil_2021} relies on a combination of automated measures and crowd-sourced verification/ \cite{li_vqa-e_2018} relies purely on automated measures but their NLEs are of low quality \cite{marasovic_natural_2020}. No NLE datasets exist for medical imaging datasets. Given the required expertise manual annotation is prohibitively expensive. We show that our automated extraction achieves very high standards, with an error rate much lower than most existing NLE datasets.
% \cite{atanasova_generating_2020} generate extractive NLEs from fact-checking documents. Using a cross-stitch layer based multi-task architecture, they show that, extracting explanations simultaneously to classifying the veracity of claims, can improve performance. 
% In CoS-E \cite{rajani_explain_2019} it is shown that they can improve performance on a commonsense question answering task by training a model to generate explanations based on the question and answer choices and then training a separate model to provide the answer given the question, answer choices, and predicted explanations. In WT5 \cite{narang_wt5_2020} they train a text-to-text model to both solve the task and generate the explanation.
% \cite{majumder_rationale-inspired_2021} combines NLEs with extractive rationales and commonsense knowledge. Their model simultaneously learns to extract rationales, augments them with commonsense knowledge, and then generate explanations based on those augmented extractive rationales. They achieve state-of-the-art (SOTA) across a range of NLP and VL tasks. 
% One of the first architectures that can provide NLEs in vision tasks is PJ-X \cite{park_multimodal_2018}, which learns a multimodal, attention-weighted representation of the input image and text (e.g., a question). An LSTM-based decoder~\cite{hochreiter_long_1997} then generates an explanation from the multimodal representation, attention map, and answer. 
% In \cite{li_vqa-e_2018}, the answer and explanation are generated simultaneously. 
% The model FME by~\cite{wu_faithful_2019} uses the UpDown architecture~\cite{anderson_bottom-up_2018} as a backbone for obtaining the multimodal representation of the input, which, together with the answer, is fed to a LSTM explanation generator. \cite{marasovic_natural_2020} use either an object detector, a situation recognition model, or VisualComet \cite{park_visualcomet_2020} as backbone, and then generate the explanation using GPT-2, a pretrained language model \cite{radford_language_nodate}. However, they do not predict the answers for task itself, but condition the explanations on the ground-truth answer. Their visual representation of the image is not trained, but fixed. 

\subsubsection{Textual Explanations in Medical Imaging.}

There has been previous work that augmented medical image classification with textual information. \cite{gale_producing_2018} designed a model that accompanies a hip fracture classification with a template-like explanation that indicates the location, severity, and type of fracture. The explanations were manually annotated by a radiologist (as the reports were deemed too inconsistent in their structure). They show that doctors prefer natural language explanations over saliency maps. \cite{lee_generation_2019} design a CNN and RNN attention-based architecture to train a model that is able to classify a mass in breast mammograms as benign or malign and provide textual explanations. The textual explanations were trained on sentences that the authors generated using the BI-RADS mass lexicons. They evaluate the sentences via automatic NLG metrics, but do not provide classification performance nor a clinical validation of the explanations. \cite{kougia_rtex_2021} proposes the RTEX system to rank and classify reports and propose natural language text to accompany the label. Their approach consists in retrieving the most similar report from the training set, using cosine similarity of the feature vector of the images and ensuring report contains the same labels as were detected in the image. That report is then used as a diagnostic sentence. Their texts have lower NLG scores than early image captioning models.
The above methods generally don't consider textual information to \emph{explain} a diagnosis, instead it only provides additional information about it. Furthermore, they all rely on template-like sentence structures, which limits their application beyond the specific use case and makes the approach less flexible. 
In this work we leverage free-text NLEs to shed transparency on the reasoning of the model about a diagnosis and equally leverage the rich information in the NLEs to learn better representations of images. We expect NLEs to both provide additional details about a diagnosis (e.g. location or severity), the degree of certainty of a diagnosis, as well as explaining how it relates to other findings and what is its evidence.

